Observation of $\eta_c(1S)\to \Sigma^0\bar \Sigma^0$ and search for $h_c(1P)\to \Sigma^0\bar \Sigma^0$ via $\psi(3686)$ transitions

Using $(2712.4 \pm 14.3) \times 10^6~\psi(3686)$ events collected by the BESIII detector operating at the BEPCII collider, the hadronic decay $\eta_{c}\to\Sigma^{0}\bar{\Sigma^{0}}$ is observed for the first time via the radiative transition from $\psi(3686)$. It is found that the branching fraction has a significant dependence on the interference pattern between $\eta_c(1S)$ and non-$\eta_c(1S)$ processes. They are determined to be $\displaystyle\mathcal{B}(\eta_c(1S) \to \Sigma^{0}\bar{\Sigma^{0}}) = (2.59 \pm 0.14(stat) \pm 0.44(syst)) \times 10^{-3}$ and $(1.18 \pm 0.12(stat) \pm 0.21(syst)) \times 10^{-3}$, for the destructive and constructive interference scenarios, respectively. No significant signal is observed for the decay $h_{c}\to\Sigma^{0}\bar{\Sigma^{0}}$ in the hadronic transition $\psi(3686)\to\pi^0h_{c}$, and an upper limit on its branching fraction is set to be $1.02\times 10^{-4}$ at the 90\% confidence level.

==> bibitem.tex <==
\begin{thebibliography}{99}

%%%%%%%%%%%%   -- Ref 1
\bibitem{Ref_a}N. Brambilla $et$ $al$., \href{https://link.springer.com/article/10.1140/epjc/s10052-010-1534-9}{Eur. Phys.J. C {\bf 71}, 1534 (2011)}.

%%%%%%%%%%%%   -- Ref 2
\bibitem{Ref_b}S.-K. Choi $et$ $al$. (Belle collaboration), \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.89.102001}{Phys. Rev. Lett. {\bf 89}, 102001 (2002)}.

%%%%%%%%%%%%   -- Ref 3
\bibitem{Ref_c}B. Aubert $et$ $al$. (BaBar collaboration), \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.92.142002}{Phys. Rev. Lett. {\bf 92}, 142002 (2004)}.

%%%%%%%%%%%%   -- Ref 4
\bibitem{Ref_d}D. M. Asner $et$ $al$. (CLEO collaboration), \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.92.142001}{Phys. Rev. Lett. {\bf 92}, 142001 (2004)}.

%%%%%%%%%%%%   -- Ref 6
\bibitem{Ref_g}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.109.042003}{Phys. Rev. Lett. {\bf 109}, 042003 (2012)}.

%%%%%%%%%%%%   -- Ref
\bibitem{Ref_06}T. Appelquist and H. D. Politzer, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.34.43}{Phys. Rev. Lett. {\bf 34}, 43 (1975)}.

%%%%%%%%%%%%   -- Ref
\bibitem{Ref_rhopi}Brodsky, Stanley J. and Lepage, G. Peter and Tuan, S. F., \href{https://doi.org/10.1103/PhysRevLett.59.621}{Phys. Rev. Lett. {\bf 59}, 621 (1987)}.

%%%%%%%%%%%%   -- Ref 12
\bibitem{Ref_09}M. Anselmino, M. Genovese, and E. Predazzi, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.44.1597}{Phys. Rev. D. {\bf 44}, 1597 (1991)}.

%%%%%%%%%%%%   -- Ref 13
\bibitem{Ref_10}K. T. Chao, Y. F. Gu, and S. F. Tuan, \href{https://iopscience.iop.org/article/10.1088/0253-6102/25/4/471}{Commun. Theor. Phys. {\bf 25}, 471 (1996)}.

%%%%%%%%%%%%   -- Ref 14
\bibitem{Ref_11}H. P. Wang and C. Z. Yuan, \href{https://doi.org/10.1088/1674-1137/ac5fa2}{Chin. Phys. C {\bf 46} 071001 (2022)}.

%%%%%%%%%%%%   -- Ref 7
\bibitem{Ref_02}S. Navas $et$ $al$. (Particle Data Group), \href{https://pdg.lbl.gov/index-2024.html}{to be published in Phys. Rev. D. {\bf 110}, 030001 (2024)}.

%%%%%%%%%%%%   -- Ref 
\bibitem{Ref_04}R. E. Mitchell $et$ $al$. (CLEO collaboration), \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.102.011801}{Phys. Rev. Lett. {\bf 106}, 159903 (2011)}.

%%%%%%%%%%%%   -- Ref 
\bibitem{Ref_05}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.108.222002}{Phys. Rev. Lett. {\bf 108}, 222002 (2012)}.

%%%%%%%%%%%%   -- Ref 
\bibitem{Ref_03}V. V. Anashin $et$ $al$., \href{https://www.sciencedirect.com/science/article/pii/S0370269314007229}{Phys. Lett. B. {\bf 738}, 391 (2014)}.

%%%%%%%%%%%%   Ref 
\bibitem{Ref_hf1s1}T. Burch $et$ $al$., \href{https://doi.org/10.1103/PhysRevD.81.034508}{Phys. Rev. D. {\bf 81}, 034508 (2010)}.

%%%%%%%%%%%%   Ref 
\bibitem{Ref_hf1s2}T. Kawanai and S. Sasaki, \href{https://doi.org/10.1103/PhysRevD.85.091503}{Phys. Rev. D. {\bf 85}, 091503 (2012)}.

%%%%%%%%%%%%   -- Ref
\bibitem{cheny} R. Q. Zhang $et$ $al$., \href{https://doi.org/10.1016/j.physletb.2022.136960}{Phys. Lett. B. {\bf 827}, 136960  (2022)}.

%%%%%%%%%%%%%%%%   Ref 
\bibitem{Ref_16}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://doi.org/10.48550/arXiv.2403.06766}{arXiv:2403.06766v3}.

%%%%%%%%%%%%   -- Ref 15
\bibitem{besiii}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://doi.org/10.1016/j.nima.2009.12.050}{Nucl. Instrum. and Meth. in Phys. Res. Sect. A. {\bf 614}, 345 (2010)}.

%%%%%%%%%%%%   -- Ref
\bibitem{besiii2}K.-X. Huang $et$ $al$., \href{https://doi.org/10.1007/s41365-022-01133-8}{Nucl. Sci. Tech. {\bf 33}, 142 (2022)}.

%%%%%%%%%%%%   -- Ref 16
\bibitem{bepcii} C.~H.~Yu {\it et al.}, \href{https://accelconf.web.cern.ch/ipac2016/talks/tuya01_talk.pdf}{Proceedings of IPAC2016, Busan, Korea, 2016, doi:10.18429/JACoW-IPAC2016-TUYA01}.

%%%%%%%%%%%%   -- Ref 17
\bibitem{etof1} X.~Li {\it et al.}, \href{https://link.springer.com/article/10.1007/s41605-017-0014-2}{Rad. Det. Tech. Meth. {\bf 1}, 13 (2017)}. 

%%%%%%%%%%%%   -- Ref 18
\bibitem{etof2} Y.~X.~Guo {\it et al.}, \href{https://link.springer.com/article/10.1007/s41605-017-0012-4}{Rad. Det. Tech. Meth. {\bf 1}, 15 (2017)}.

%%%%%%%%%%%%   -- Ref 19
\bibitem{etof3} P.~Cao {\it et al.}, \href{https://dx.doi.org/10.1016/j.nima.2019.163053}{Nucl. Instrum. and Meth. in Phys. Res. Sect. A. {\bf 953}, 163053 (2020)}.

%%%%%%%%%%%%   -- Ref 20
\bibitem{G4} S. Agostinelli $et$ $al$. (GEANT4 collaboration), \href{https://www.sciencedirect.com/science/article/abs/pii/S0168900203013688}{Nucl. Instrum. and Meth. in Phys. Res. Sect. A. {\bf 506}, 250 (2003)}.

%%%%%%%%%%%%   -- Ref 21
\bibitem{kkmc} S.~Jadach, B.~F.~L.~Ward and Z.~Was, \href{https://doi.org/10.1103/PhysRevD.63.113009}{Phys. Rev. D 63, 113009(2001)}; \href{https://doi.org/10.1016/S0010-4655(00)00048-5}{Comput. Phys. Commun., {\bf 130}, 260 (2000)}.

%%%%%%%%%%%%   -- Ref
\bibitem{evtgen1} D. J.~Lange, \href{https://dx.doi.org/10.1016/S0168-9002(01)00089-4}{Nucl. Instrum. and Meth. in Phys. Res. Sect. A. {\bf 462}, 152 (2001)}.

%%%%%%%%%%%%   -- Ref 
\bibitem{evtgen2} R. G.~Ping, \href{https://doi.org/10.1088/1674-1137/32/8/001}{Chin. Phys. C {\bf 32} 599 (2008)}.

%%%%%%%%%%%%   -- Ref 24
\bibitem{lundcharm1} J. C. Chen, G. S. Huang, X. R. Qi, D. H. Zhang and Y. S. Zhu, \href{https://doi.org/10.1103/PhysRevD.62.034003}{Phys. Rev. D {\bf 62}, 034003(2000)}.

%%%%%%%%%%%%   -- Ref 25
\bibitem{lundcharm2} R. L. Yang, R. G. Ping, and H. Chen, \href{https://iopscience.iop.org/article/10.1088/0256-307X/31/6/061301}{Chin.\ Phys.\ Lett. {\bf 31}, 061301 (2014)}.

%%%%%%%%%%%%   -- Ref
\bibitem{fsr} E. Barberio and Z. Was, \href{https://doi.org/10.1016/0010-4655(94)90074-4}{Comput.\ Phys.\ Commun. {\bf 79}, 291 (1994)}.

%%%%%%%%%%%%%%%%   Ref 27
\bibitem{Ref_12}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.106.032014}{Phys. Rev. D. {\bf 106}, 032014 (2022)}.

%%%%%%%%%%%%   Ref
\bibitem{Ref_topo}X. Y. Zhou  $et$ $al$. \href{https://doi.org/10.1016/j.cpc.2020.107540}{Comput. Phys. Commun. {\bf 258}, 107540 (2021)}.

%%%%%%%%%%%%%%%%   Ref
\bibitem{etac2s3}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://doi.org/10.1103/PhysRevD.107.052007}{Phys. Rev. D {\bf 107}, 052007 (2023)}.

%%%%%%%%%%%%%%%%   Ref
\bibitem{etac2s1}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://doi.org/10.1103/PhysRevLett.109.042003}{Phys. Rev. Lett. {\bf 109}, 042003 (2012)}.

%%%%%%%%%%%%%%%%   Ref
\bibitem{etac2s2}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://doi.org/10.1103/PhysRevD.87.052005}{Phys. Rev. D {\bf 87}, 052005 (2013)}.

%%%%%%%%%%%%   Ref 28
\bibitem{Ref_13}V. V. Anashin $et$ $al$., \href{https://arxiv.org/abs/1012.1694}{arXiv: 1012.1694}.

%%%%%%%%%%%%   Ref
\bibitem{Ref_arg}H. Albrecht $et$ $al$. (ARGUS collaboration), \href{https://doi.org/10.1016/0370-2693(90)91293-K}{Phys. Lett. B {\bf 241}, 278 (1990)}.

%%%%%%%%%%%%   Ref 
\bibitem{Ref_18}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://doi.org/10.1103/PhysRevD.87.012002}{Phys. Rev. D. {\bf 87}, 012002 (2013)}.

%%%%%%%%%%%%%%%%   Ref 29
\bibitem{Ref_14}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://doi.org/10.1103/PhysRevD.83.112005}{Phys. Rev. D {\bf 83}, 112005(2011)}.

%%%%%%%%%%%%%%%%   Ref 30
\bibitem{Ref_15}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.81.052005}{Phys. Rev. D {\bf 81}, 052005(2010)}.

%%%%%%%%%%%%%%%%   Ref 32
\bibitem{Ref_19}M. Ablikim $et$ $al$. (BESIII collaboration), \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.100.012003}{Phys. Rev. D {\bf 100}, 012003 (2019)}.

%%%%%%%%%%%%%%%%   Ref
\bibitem{Ref_mixing1}Y. D. Tsai $et$ $al$., \href{https://doi.org/10.1103/PhysRevD.85.034002}{Phys. Rev. D {\bf 85}, 034002 (2012)}.

%%%%%%%%%%%%%%%%   Ref
\bibitem{Ref_mixing2}W. Qin $et$ $al$., \href{https://doi.org/10.1103/PhysRevD.97.096002}{Phys. Rev. D {\bf 97}, 096002 (2018)}.

%%%%%%%%%%%%%%%%   Ref loop
\bibitem{loop} Q. Wang  $et$ $al$. \href{https://doi.org/10.1016/j.physletb.2012.04.022}{Phys. Lett. B {\bf 711}, 364370 (2012)}.

\end{thebibliography}
